Uncovering the New Accessibility Crisis in Scholarly PDFs

Most scholarly works are distributed online in PDF format, which can present significant accessibility challenges for blind and low-vision readers. To characterize the scope of this issue, we perform a large-scale analysis of 20K open- and closed-access scholarly PDFs published between 2014-2023 sampled across broad fields of study. We assess the accessibility compliance of these documents based on six criteria: Default Language, Appropriate Nesting, Tagged PDF, Table Headers, Tab Order, and Alt-Text; selected based on prior work and the SIGACCESS Guide for Accessible PDFs. To ensure robustness, we corroborate our findings through automated accessibility checking, manual evaluation of alt text, comparative assessments with an alternate accessibility checker, and manual assessments with screen readers. Our findings reveal that less than 3.2% of tested PDFs satisfy all criteria, while a large majority (74.9%) fail to meet any criteria at all. Worse yet, we observe a concerning drop in PDF accessibility since 2019, largely among open-access papers, suggesting that efforts to improve document accessibility have not taken hold and are on a backslide. While investigating factors contributing to this drop, we identify key associations between fields of study, creation platforms used, models of publishing, and PDF accessibility compliance, suggesting that publisher and author choices significantly influence document accessibility. This paper highlights a new crisis in scholarly document accessibility and the need for a multi-faceted approach to address the problem, involving the development of better tools, enhanced author education, and systemic changes in academic publishing practices.

==> figtabs/fig_compliance_model_time.tex <==
\begin{figure}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figures/compliance_model_time.png}
  \caption{
  Accessibility compliance for models of publishing over time (2014-2023). There is a significant decline in mean normalized total compliance during 2017-2020 for open access papers. Following this, the compliance values remain stable or increase slightly. \lucy{add error bars if easy -- standard error}}
  \label{fig:compliance_model_time}
  % \Description{A line plot shows the proportion of different typesetting software in our sample between 2010-2019. Microsoft Word, Adobe InDesign, and LaTeX have all increased in proportional usage (all starting at a proportion of 0.07-0.08 in 2010 to 0.15 or above in 2019. The usage of printer drivers to create PDFs has declined from a proportion of 0.12 in 2010 to around 0.05 in 2019. Arbortext APP also shows a modest decline in recent years to below a proportion 0.10.}
\end{figure}

==> figtabs/fig_compliance_model_time_errors.tex <==
\begin{figure}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figures/compliance_model_time_errors.png}
  \caption{
  Accessibility compliance for models of publishing over time (2014-2023) with error bars. There is a significant decline in mean normalized total compliance during 2017-2020 for open access papers. Following this, the compliance values remain stable or increase slightly.}
  \label{fig:compliance_model_time_errors}
  % \Description{A line plot shows the proportion of different typesetting software in our sample between 2010-2019. Microsoft Word, Adobe InDesign, and LaTeX have all increased in proportional usage (all starting at a proportion of 0.07-0.08 in 2010 to 0.15 or above in 2019. The usage of printer drivers to create PDFs has declined from a proportion of 0.12 in 2010 to around 0.05 in 2019. Arbortext APP also shows a modest decline in recent years to below a proportion 0.10.}
\end{figure}

==> figtabs/fig_latex_by_fos.tex <==
\begin{figure}[t!]
  \centering
    \includegraphics[width=0.64\linewidth]{figures/prop_latex_vs_compliance_by_fos.png}
  \caption{There is a strong negative correlation ($r = -0.74$, $p < 0.001$, 95\% CI shown) between the proportion of PDFs typeset using LaTex and the mean normalized Total Compliance of papers by field of study. Fields such as Mathematics, Physics, and Computer science use LaTeX around or over 15\% of the time, and have correspondingly lower mean accessibility compliance. On the other end of the spectrum are fields like Medicine and Environment science, where LaTeX is rarely used, and which have very high levels of mean compliance.}
  \label{fig:prop_latex_by_fos}
  \Description{A scatter plot shows a negative correlation between the proportion of PDFs typeset using LaTeX and the mean normalized total compliance score by field of study. Fields that typeset more using LaTeX have lower Total Compliance scores. The correlation coefficient r is -0.74, and p is less than 0.001. Fields that use LaTeX more and have lower compliance rates include Mathematics, Physics, and Computer science. Fields that use LaTeX very little and have high compliance rates include Medicine and Environment science.}
\end{figure}

==> figtabs/fig_prop_others_compliance.tex <==
\begin{figure*}[ht!]
  \centering
    \includegraphics[width=0.9\linewidth]{figures/prop_others_compliance.png}
  \caption{Correlation between PDF Creation Software Usage and Accessibility Compliance by Field of Study. The figure shows a positive correlation between the proportion of PDFs created using Elsevier and their accessibility compliance (r = 0.53, p < 0.05, 95\% CI), while correlations for Adobe InDesign, Springer, and XPP are non-significant (r = 0.16, 0.12, and -0.06 respectively, all non-significant)}
  \label{fig:prop_others_compliance}
  \Description{Four scatter plots show the correlation between the proportion of PDFs created by different platforms (Adobe InDesign, XPP, Elsevier, and Springer) and their mean normalized total compliance scores across various fields of study. The plot shows a significant positive correlation for PDFs created using Elsevier (correlation coefficient r is 0.53, p less than 0.05, 95\% Confidence Interval), whereas correlations for PDFs from Adobe InDesign, Springer, and XPP are not significant (correlation coefficients r = 0.16, 0.12, and -0.06, respectively).}
\end{figure*}

==> figtabs/fig_prop_software_compliance.tex <==
\begin{figure}[t!]
  \centering
    \includegraphics[width=0.76\linewidth,trim={5mm 10mm 3mm 10mm},clip]{figures/prop_software_compliance.png}
  \caption{There are significant and contrasting correlations between the proportion of PDFs created using Microsoft Word and LaTex, and the mean normalized Total Compliance of papers by field of study. Microsoft Word shows a strong positive correlation ($r = 0.66$, $p < 0.01$, 95\% CI shown) with higher compliance in fields like Medicine, Environmental Science, Business, Political Science, Sociology, Economics, and Psychology, where its usage exceeds 15\%. Conversely, LaTeX demonstrates a strong negative correlation ($r = -0.74$, $p < 0.001$, 95\% CI shown) with lower compliance, particularly in fields such as Mathematics, Physics, and Computer Science, where it is used similarly extensively. \lucy{merge with figure 11 if moving to appendix}}
  \label{fig:prop_software_compliance}
  \Description{Two scatter plots showing the correlations between the proportion of PDFs created using Microsoft Word and LaTeX, and the mean normalized total compliance score by field of study. Microsoft Word shows a positive correlation (correlation coefficient r is 0.66 and p less than 0.01) with higher compliance scores in fields like Medicine, Environmental Science, and Psychology. Conversely, LaTeX shows a negative correlation (correlation coefficient r is -0.74 and p less than p < 0.001), with higher usage correlating to lower compliance scores in fields like Mathematics, Physics, and Computer Science.}
\end{figure}




==> figtabs/fig_word_by_fos.tex <==
\begin{figure}[t!]
  \centering
    \includegraphics[width=0.64\linewidth]{figures/prop_word_vs_compliance_by_fos.png}
  \caption{There is a strong positive correlation ($r = 0.66$, $p < 0.01$, 95\% CI shown) between the proportion of PDFs typeset using Microsoft Word and the mean normalized Total Compliance of papers by field of study. Fields such as Medicine, Environment science, Business, Political science, Sociology, Economics, and Psychology use Microsoft Word around or over 15\% of the time, and have correspondingly higher mean accessibility compliance. On the other end of the spectrum are fields like Geography, Physics, and Mathematics, where Microsoft Word is used less, and which have very low levels of mean compliance. \lucy{maybe plot this and latex side by side (two subplots for easy comparison); add same plots for other typesetting softwares into the appendix}}
  \label{fig:prop_word_by_fos}
  \Description{A scatter plot shows a positive correlation between the proportion of PDFs typeset using Microsoft Word and the mean normalized total compliance score by field of study. Fields that typeset more using Word have higher Total Compliance scores. The correlation coefficient r is 0.66, and p is less than 0.01. Fields that use Word more and have higher compliance rates include Medicine, Environment science, Business, Political science, Sociology, Economics, and Psychology. Fields that use Word very little and have low compliance rates include Geography, Physics, and Mathematics.}
\end{figure}

==> figtabs/tab_chi_comparison.tex <==
\begin{table}[t!]
\begin{tabular}{lccc}
    \toprule
    \textbf{Criterion} & \textbf{CHI 2010~\citep{Lazar2017MakingTF}} & \textbf{Ours-CHI 2010} & \textbf{Ours-FOS All (19997)} \\ 
    \midrule
    Alt-text & 3.6\% & 4.0\% & 8.5\%  \\
    Table headers & 0.7\% & 1.0\% & 13.4\% \\
    Tagged PDF & 6.3\% & 7.4\% & 12.6\% \\
    Default language & 2.3\% & 3.0\% & 17.3\% \\
    Tab order & 0.3\% & 1.0\% & 6.8\% \\
    Appropriate Nesting & - & - & 15.9\% \\
    \midrule
    Adobe-6 Compliance & - & - & 3.2\% \\
    \bottomrule
\end{tabular}
\caption{We reproduce the analysis conducted by \citet{Lazar2017MakingTF} on PDFs of papers published in CHI, showing the percentage of papers that satisfy each of the five accessibility criteria. We find similar compliance rates, indicating that our automated accessibility checker pipeline is comparable to previous analysis methods. We also show the percentage of papers in our full dataset of \numpdfs PDFs that satisfy each criterion, along with the percent that satisfy \xcompliance{5}.
}
\label{tab:chi-results}
% \Description{
% Criterion; CHI 2010 [23]; Ours-CHI 2010; Ours-All (11,397)
% Alt-text; 3.6%; 4.0%; 7.5%
% Table headers; 0.7%; 1.0%; 13.3%
% Tagged PDF; 6.3%; 7.4%; 13.4%
% Default language; 2.3%; 3.0%; 17.2%
% Tab order; 0.3%; 1.0%; 9.3%
% Adobe-5 Compliance; -; -; 2.4
% }
\end{table}

% \begin{table}[t!]
% \begin{tabular}{lcccc}
%     \toprule
%     \textbf{Criterion} & \textbf{CHI 2010~\citep{Lazar2017MakingTF}} & \textbf{Ours-CHI 2010} & \textbf{Ours-CHI All (\numchitotal)} & \textbf{Ours-FOS All (\numpdfs)} \\ 
%     \midrule
%     Alt-text & 3.6\% & 4.0\% & 7.9\% & 7.5\%  \\
%     Table headers & 0.7\% & 1.0\% & 7.2\% & 13.3\% \\
%     Tagged PDF & 6.3\% & 7.4\% & 15.2\% & 13.4\% \\
%     Default language & 2.3\% & 3.0\% & 29.5\% & 17.2\% \\
%     Tab order & 0.3\% & 1.0\% & 6.5\% & 9.3\% \\
%     \midrule
%     \xcompliance{5} & - & - & 2.0\% & 2.4\% \\
%     \bottomrule
% \end{tabular}
% \caption{We reproduce the analysis conducted by \citet{Lazar2017MakingTF} on PDFs of papers published in CHI, showing the percentage of papers that satisfy each of the five accessibility criteria. We find similar compliance rates, indicating that our automated accessibility checker pipeline is comparable to previous analysis methods. We also show the percentage of papers in our full dataset of \numpdfs PDFs that satisfy each criterion, along with the percent that satisfy \xcompliance{5}.
% }
% \label{tab:chi-results}
% % \Description{
% % Criterion; CHI 2010 [23]; Ours-CHI 2010; Ours-All (11,397)
% % Alt-text; 3.6%; 4.0%; 7.5%
% % Table headers; 0.7%; 1.0%; 13.3%
% % Tagged PDF; 6.3%; 7.4%; 13.4%
% % Default language; 2.3%; 3.0%; 17.2%
% % Tab order; 0.3%; 1.0%; 9.3%
% % Adobe-5 Compliance; -; -; 2.4
% % }
% \end{table}

==> figtabs/tab_rw.tex <==
\begin{table}[t!]
\small
    \centering
    \begin{tabularx}{\linewidth}{L{22mm}L{15mm}L{48mm}L{16mm}L{34mm}}
        \toprule
        \textbf{Prior work} & \textbf{PDFs analyzed} & \textbf{Venues} & \textbf{Year} & \textbf{Accessibility checker} \\
        \midrule
        \citet{Brady2015CreatingAP} & 1,811 & CHI, ASSETS and W4A & 2011--2014 & PDFA Inspector \\ [0.5mm]
        \hline \\ [-2.5mm]
        \citet{Lazar2017MakingTF} & 465 + 32 & CHI and ASSETS & 2014--2015 & Adobe Acrobat Action Wizard \\ [0.5mm]
        \hline \\ [-2.5mm]
        \citet{Ribera2019PublishingAP} & 59 & DSAI & 2016 & Adobe PDF Accessibility Checker 2.0 \\ [0.5mm]
        \hline \\ [-2.5mm]
        \citet{Nganji2015ThePD} & 200 & \textit{Disability \& Society}, \textit{Journal of Developmental and Physical Disabilities}, \textit{Journal of Learning Disabilities}, and \textit{Research in Developmental Disabilities} & 2009--2013 & Adobe PDF Accessibility Checker 1.3 \\ [0.6mm]
        \hline \\ [-2.5mm]
        \textbf{\textit{Our analysis}} & \numpdfs & Venues across various fields of study & 2010--2019 & Adobe Acrobat Accessibility Plug-in Version 21.001.20145 \\
        \bottomrule
    \end{tabularx}
    \caption{Prior work has investigated PDF accessibility for papers published in specific venues such as CHI, ASSETS, W4A, DSAI, or various disability journals. Several of these works were conducted manually, and were limited to a small number of papers, while the more thorough analysis was conducted for CHI and ASSETS, two conference venues focused on accessibility and HCI. Our study expands on this prior work to investigate accessibility over \numpdfs PDFs sampled from across different fields of study.
    }
    % \Description{
% Prior work, PDFs analyzed, Venues, Year, Accessibility checker 
% Brady et al. [7], 1811, CHI, ASSETS and W4A, 2011--2014, PDFA Inspector 
% Lazar et al. [23], 465 + 32, CHI and ASSETS, 2014--2015, Adobe Acrobat Action Wizard 
% Ribera et al. [40], 59, DSAI, 2016, Adobe PDF Accessibility Checker 2.0 
% Nganji [33], 200, Disability & Society, Journal of Developmental and Physical Disabilities, Journal of Learning Disabilities, and Research in Developmental Disabilities, 2009--2013, Adobe PDF Accessibility Checker 1.3
% Our analysis, 11397, Venues across various fields of study, 2010--2019, Adobe Acrobat Accessibility Plug-in Version 21.001.20145 
    % }
    \label{tab:prior_work}
\end{table}

==> figtabs/tab_typesetting.tex <==
\begin{table}[t!]
\begin{tabular}{ll}
    \toprule
        \textbf{Typesetting Software} & \textbf{Count (\%)} \\ 
    \midrule
        
        Arbortext APP        & 3966 (19.8\%) \\
        Adobe InDesign       & 2892 (14.5\%) \\
        LaTeX                & 2443 (12.2\%) \\
        Microsoft Word       & 1291 (6.5\%) \\
        XPP                  & 1216 (6.1\%) \\
        Springer             & 911  (4.6\%) \\
        Elsevier             & 795  (4.0\%) \\
    \midrule
        Other                & 6483 (32.3\%) \\
    \bottomrule
\end{tabular}
\caption{Count of papers per Typesetting Software. ``Other'' includes PDFs created with an additional 22 unique software programs, each with counts of less than 350, as well as those created with unknown typesetting software. \lucy{Can we combine these counts into Figure 5?}}
\label{tab:dist-of-headers}
% \Description{
% Typesetting Software; Count (%)
% Adobe InDesign; 1591 (14.0%)
% LaTeX; 1431 (12.6%)
% Arbortext APP; 1374 (12.1%)
% Microsoft Word; 1318 (11.6%)
% Printer; 1021 (9.0%)
% Other; 4662 (40.9%)
% }
\end{table}
